Input Resolution Downsizing as a Compression Technique for Vision Deep Learning Systems

Model compression is a critical area of research in deep learning, in particular in vision, driven by the need to lighten models memory or computational footprints. While numerous methods for model compression have been proposed, most focus on pruning, quantization, or knowledge distillation. In this work, we delve into an under-explored avenue: reducing the resolution of the input image as a complementary approach to other types of compression. By systematically investigating the impact of input resolution reduction, on both tasks of classification and semantic segmentation, and on convnets and transformer-based architectures, we demonstrate that this strategy provides an interesting alternative for model compression. Our experimental results on standard benchmarks highlight the potential of this method, achieving competitive performance while significantly reducing computational and memory requirements. This study establishes input resolution reduction as a viable and promising direction in the broader landscape of model compression techniques for vision applications.

==> figures/Autres/brouillon.tex.tex <==
To enhance the accuracy of CNNs at lower resolutions and further compress model inference, we propose two techniques inspired by \cite{touvronFixingTraintestResolution2022}:
\begin{itemize}
    \item Reduce the random crop size used during training.
    \item Keep the random crop size at a higher resolution and resizing it to a lower resolution after the first convolutional layer.
\end{itemize}
% maths 1

The optimization problem for the first method can be formalized as follows: Given a CNN $N$ consisting of $s$ layers $F_i$, $i \in \{1, \dots, s\}$, and an input tensor $x \in \mathbb{R}^{3 \times R}$, where $R$ represents the resolution of the input image, the network is defined as:
\begin{equation} \label{eq:defCNN}
    \begin{aligned}
        & N(x) = (\bigodot_{i=1,...,s}{F_{i}}) (x)
    \end{aligned}
\end{equation}
The objective is to maximize the accuracy of $N$ under specific memory and computational constraints:
\begin{equation} \label{eq:defCNN2}
    \begin{aligned}
    & \underset{K_{train}, K_{crop}, K}{\text{max}}\text{ }  {  Accuracy}(N) \\
    & \text{s.t.  }\text{Memory}(N) \leq \text{target memory}, \\
    & \text{Ops}(N) \leq \text{target ops}
    \end{aligned}
\end{equation}
To solve this optimization problem, we perform a grid search. Since optimizing for $K_{eval}$ and $K$ requires only evaluating the model post-training, the search space for these parameters can be more detailed than for $K_{train}$. Additionally, as noted by \cite{touvronFixingTraintestResolution2022}, due to differences between training and evaluation data augmentations, a network trained with a random crop size $K_{train}$ tends to achieve peak accuracy when $K_{crop} \geq K_{train}$.

For the second method proposed, we introduce a resize layer $R$ during training, defined as: 
\begin{align}
    R : \left|
        \begin{array}{ll}
            x & \longrightarrow  \text{downscaling(x)} \\
            \mathbb{R}^{C\times R_{1}^{2}} & \longrightarrow \mathbb{R}^{C\times R_{2}^{2}}
        \end{array}
    \right.
\end{align}
The convolutional neural network can be redefined :
\begin{equation} \label{eq:defmethod2}
    \begin{aligned}
    N(x) = \left|
        \begin{array}{ll}
            (\underset{i=2,...,s}{\bigodot}{F_{i}}) (R \circ F_1(x)) & \text{in training} \\
            (\underset{i=1,...,s}{\bigodot}{F_{i}}) (x) & \text{in evaluation}
        \end{array}
    \right.
    \end{aligned}
\end{equation}
with C as the number of channels defined by the previous convolutional layer and $R_{1}, R_{2} \in \mathbb{R}$ and $R_{1} \geq R_{2}$, The optimization objective become :
\begin{equation} \label{eq:defCNN3}
    \begin{aligned}
    & \underset{K_{train}, K_{crop}, K, R_2}{\text{max}}\text{ }  {  Accuracy}(N) \\
    \end{aligned}
\end{equation}

==> figures/RegSeg0/regseg0_2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
title={RegSeg Resolution Scaling Methods},
x grid style={darkgray176},
xlabel={Complexity (size of crops)},
xmajorgrids,
xmin=57.6, xmax=1606.4,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Cityscapes mIoU},
ymajorgrids,
ymin=65, ymax=79,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180, dotted, mark=*, mark size=3.5, mark options={solid}]
table {%
128 49.83
256 63.65
384 69.43
512 72.2
640 73.07
768 72.9
896 72.34
1024 71.34
1280 64.98
1536 54.24
};
\addlegendentry{$FCR_256$}
\addplot [semithick, darkorange25512714, dotted, mark=*, mark size=3.5, mark options={solid}]
table {%
128 39.65
256 60.72
384 68.12
512 72.23
640 74.65
768 75.91
896 76.39
1024 76.21
1280 75.68
1536 74.32
};
\addlegendentry{$FCR_384$}
\addplot [semithick, forestgreen4416044, dotted, mark=*, mark size=3.5, mark options={solid}]
table {%
128 40.13
256 59.88
384 68.01
512 72.58
640 74.87
768 76.3
896 77.4
1024 77.87
1280 78.1
1536 77.53
};
\addlegendentry{$768_400_1600$}
\addplot [semithick, crimson2143940, dotted, mark=*, mark size=3.5, mark options={solid}]
table {%
128 44.53
256 63.02
384 70.24
512 74.17
640 75.99
768 76.81
896 77.26
1024 77.26
1280 76.32
1536 74.41
};
\addlegendentry{$768_300_1200$}
\addplot [semithick, mediumpurple148103189, dotted, mark=*, mark size=3.5, mark options={solid}]
table {%
128 44.38
256 60.16
384 66.71
512 71.21
640 73.58
768 75.24
896 76.22
1024 76.55
1280 76.05
1536 74.81
};
\addlegendentry{$512_400_1600$}
\addplot [semithick, sienna1408675, dotted, mark=*, mark size=3.5, mark options={solid}]
table {%
128 50.48
256 65.11
384 70.31
512 73.17
640 74.07
768 73.98
896 73.29
1024 71.88
1280 67.52
1536 58.3
};
\addlegendentry{$512_200_800$}
\end{axis}

\end{tikzpicture}


==> figures/VIT0/test.tex <==
% \documentclass{standalone}
% \pgfplotsset{compat = newest}



% \begin{document}
% This file was created with tikzplotlib v0.10.1.
\resizebox{0.5\textwidth}{!}
{
    {
\begin{tikzpicture}
\definecolor{Paired_4}{RGB}{44,160,44}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{fu-blue}{RGB}{0, 51, 102} % blue text
\definecolor{fu-green}{RGB}{153, 204, 0} % green text	        % group style={
        %     % set how the plots should be organized
        %     group size=1 by 2,
        %     % only show ticklabels and axis labels on the bottom
        %     x descriptions at=edge bottom,
        %     % set the `vertical sep' to zero
        %     vertical sep=0pt,
        % },
\begin{groupplot}[group style={group size=2 by 1,
                                horizontal sep=0pt},
                                % xlabels at=edge bottom,  % Place xlabel at the bottom edge
                                % xticklabels at=edge bottom, % Only show xtick labels at the bottom edge
                  ]
\nextgroupplot[
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.03,0.97)},
      anchor=north west,
      draw=darkgray176,
     legend columns=2
    },
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=4600000000, xmax=4900000000,
xtick style={color=black},
y grid style={darkgray176},
ymin=67, ymax=74,
ytick style={color=black},
axis y line=left,
xmajorgrids,
ymajorgrids,
xtick={4.6e9, 4.7e9, 4.8e9, 4.85e9},
xticklabels={4.6, 4.7, 4.8, 4.85},
scaled x ticks=false,
ylabel={ImageNet Top-1(\%)},
scaled x ticks=false,
xlabel={Computational Cost (GFLOPs)},
x label style={at={(axis description cs:1,-0.1)},anchor=north},
 % xlabel={FLOPS}
]
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=triangle*, only marks] table [x=ps8a, y=ps8b,col sep=comma]   {figures/VIT0/points.csv};\label{patate}
    % \addlegendentry{Patch Size $8$}
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=*, only marks] table [x=ps12a, y=ps12b,col sep=comma]   {figures/VIT0/points.csv};\label{plot:ps12}
    % \addlegendentry{Patch Size $12$}
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=diamond*, only marks] table [x=ps16a, y=ps16b,col sep=comma]   {figures/VIT0/points.csv};\label{plot:ps16}
    % \addlegendentry{Patch Size $16$}
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=square*, only marks] table [x=ps24a, y=ps24b,col sep=comma]   {figures/VIT0/points.csv};\label{plot:ps24}
    % \addlegendentry{Patch Size $24$}
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=pentagon*, only marks] table [x=ps32a, y=ps32b,col sep=comma]   {figures/VIT0/points.csv};\label{plot:ps32}
    % \addlegendentry{Patch Size $32$}
    \addplot [draw=Paired_5, fill=Paired_5, mark size=3, mark=*, only marks] table [x=a, y=b,col sep=comma]   {figures/VIT0/MLPscaling.csv};\label{plot:mlp0}
    % \addlegendentry{MLP scaling}
    \addplot [draw=Paired_1, fill=Paired_1, mark size=3, mark=*, only marks] table [x=a, y=b,col sep=comma]   {figures/VIT0/HDscaling.csv};\label{plot:hd0}
    % \addlegendentry{HD Scaling}
    \addplot [draw=Paired_5, fill=Paired_5, mark size=3, mark=*, only marks] table [x=c, y=d,col sep=comma]   {figures/VIT0/MLPscaling.csv};
    \addplot [semithick, black, dashed] table [x=a, y=b,col sep=comma]  {figures/VIT0/test.csv};
\nextgroupplot[
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={darkgray176},
xmin=8800000000, xmax=9350000000,
xtick pos=left,
xtick style={color=black},
y grid style={darkgray176},
ymin=67, ymax=74,
ytick pos=right,
ytick style={color=black},
yticklabels={},
axis x discontinuity=parallel,
axis y line=right,
xmajorgrids,
ymajorgrids,
xtick={8.8e9, 8.9e9, 9e9, 9.1e9, 9.2e9, 9.3e9},
xticklabels={, 8.9, 9, 9, 9.1, 9.2, 9.3},
scaled x ticks=false,
]
    \addplot [draw=Paired_1, fill=Paired_1, mark size=3, mark=*, only marks] table [x=c, y=d,col sep=comma]   {figures/VIT0/HDscaling.csv};
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=triangle*, only marks] table [x=ps8c, y=ps8d,col sep=comma]   {figures/VIT0/points.csv};
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=*, only marks] table [x=ps12c, y=ps12d,col sep=comma]   {figures/VIT0/points.csv};
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=diamond*, only marks] table [x=ps16c, y=ps16d,col sep=comma]   {figures/VIT0/points.csv};
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=square*, only marks] table [x=ps24c, y=ps24d,col sep=comma]   {figures/VIT0/points.csv};
    \addplot [draw=Paired_4, fill=Paired_4, mark size=3, mark=pentagon*, only marks] table [x=ps32c, y=ps32d,col sep=comma]   {figures/VIT0/points.csv};
    \addplot [draw=Paired_5, fill=Paired_5, mark size=3, mark=*, only marks] table [x=e, y=f,col sep=comma]   {figures/VIT0/MLPscaling.csv};
    \addplot [semithick, black, dashed] table [x=c, y=d,col sep=comma]  {figures/VIT0/test.csv};

\coordinate (legend) at (axis description cs:-1.0,1.0);
\end{groupplot}

\matrix [
    draw,
    matrix of nodes,
    anchor=north west,
    fill=white,
    row sep=-4pt,
    column sep=-6pt,
] at (legend) {
    \pgfmatrixnextcell [-10pt ]Patch Size  \pgfmatrixnextcell [5pt]\pgfmatrixnextcell     [5pt]           \\
    \ref{patate} \pgfmatrixnextcell 8 \pgfmatrixnextcell \ref{plot:mlp0}  \pgfmatrixnextcell MLP Scaling\\
    \ref{plot:ps12} \pgfmatrixnextcell 12 \pgfmatrixnextcell \ref{plot:hd0}  \pgfmatrixnextcell HD Scaling\\
    \ref{plot:ps16} \pgfmatrixnextcell 16 \pgfmatrixnextcell \\
    \ref{plot:ps24} \pgfmatrixnextcell 24 \pgfmatrixnextcell \\
    \ref{plot:ps32} \pgfmatrixnextcell 32 \pgfmatrixnextcell \\
};
\end{tikzpicture}
}}
% \end{document}
